How Do Static and Dynamic Test Case Prioritization Techniques Perform on Modern Software Systems? An Extensive Study on GitHub Projects

Test Case Prioritization (TCP) is an increasingly important regression testing technique for reordering test cases according to a pre-defined goal, particularly as agile practices gain adoption. To better understand these techniques, we perform the first extensive study aimed at empirically evaluating four static TCP techniques, comparing them with state-of-research dynamic TCP techniques across several quality metrics. This study was performed on 58 real-word Java programs encompassing 714 KLoC and results in several notable observations. First, our results across two effectiveness metrics (the Average Percentage of Faults Detected APFD and the cost cognizant APFDc) illustrate that at test-class granularity, these metrics tend to correlate, but this correlation does not hold at test-method granularity. Second, our analysis shows that static techniques can be surprisingly effective, particularly when measured by APFDc. Third, we found that TCP techniques tend to perform better on larger programs, but that program size does not affect comparative performance measures between techniques. Fourth, software evolution does not significantly impact comparative performance results between TCP techniques. Fifth, neither the number nor type of mutants utilized dramatically impact measures of TCP effectiveness under typical experimental settings. Finally, our similarity analysis illustrates that highly prioritized test cases tend to uncover dissimilar faults.

==> evolution.tex <==
\begin{figure*}
 \center
\begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/JActor-APFD-Method.png}
 \caption{TCP results on JActor (APFD)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/JActor-APFDC-Method.png}
 \caption{TCP results on JActor (APFDC)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/LastCalc-APFD-Method.png}
 \caption{TCP results on LastCalc (APFD)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/LastCalc-APFDC-Method.png}
 \caption{TCP results on LastCalc (APFDC)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/gdx-artemis-APFD-Method.png}
 \caption{TCP results on gdx-artemis (APFD)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/gdx-artemis-APFDC-Method.png}
 \caption{TCP results on gdx-artemis (APFDC)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/geojson-jackson-APFD-Method.png}
 \caption{TCP results on geojson-jackson (APFD)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/geojson-jackson-APFDC-Method.png}
 \caption{TCP results on geojson-jackson (APFDC)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/gson-fire-APFD-Method.png}
 \caption{TCP results on gson-fire (APFD)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/gson-fire-APFDC-Method.png}
 \caption{TCP results on gson-fire (APFDC)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/jackson-dataformat-xml-APFD-Method.png}
 \caption{TCP results on jackson-dataformat-xml (APFD)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/jackson-dataformat-xml-APFDC-Method.png}
 \caption{TCP results on jackson-dataformat-xml (APFDC)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/jackson-datatype-joda-APFD-Method.png}
 \caption{TCP results on jackson-datatype-joda (APFD)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/jackson-datatype-joda-APFDC-Method.png}
 \caption{TCP results on jackson-datatype-joda (APFDC)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/javapoet-APFD-Method.png}
 \caption{TCP results on javapoet (APFD)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/javapoet-APFDC-Method.png}
 \caption{TCP results on javapoet (APFDC)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/jprotobuf-APFD-Method.png}
 \caption{TCP results on jprotobuf (APFD)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/jprotobuf-APFDC-Method.png}
 \caption{TCP results on jprotobuf (APFDC)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/protoparser-APFD-Method.png}
 \caption{TCP results on protoparser (APFD)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/protoparser-APFDC-Method.png}
 \caption{TCP results on protoparser (APFDC)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/pusher-websocket-java-APFD-Method.png}
 \caption{TCP results on pusher-websocket-java (APFD)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/pusher-websocket-java-APFDC-Method.png}
 \caption{TCP results on pusher-websocket-java (APFDC)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/stateless4j-APFD-Method.png}
 \caption{TCP results on stateless4j (APFD)}
 \end{subfigure}
 \begin{subfigure}{0.48\textwidth}
 \captionsetup{skip=-3pt}
 \includegraphics[scale=0.25]{boxplots/stateless4j-APFDC-Method.png}
 \caption{TCP results on stateless4j (APFDC)}
 \end{subfigure}
 \caption{\label{fig:ev} Method-level test prioritization in evolution}
\end{figure*}


==> macro.tex <==
\usepackage{subcaption}
\usepackage{url}
\usepackage{amssymb}
\usepackage{ifthen}
\usepackage{amsmath}
\usepackage{comment}
%\usepackage{subfig}

\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }




\newcommand\KEVIN[1]{\nb{KEVIN}{#1}}
\newcommand\DENYS[1]{\nb{DENYS}{#1}}
\newcommand\QI[1]{\nb{QI}{#1}}
\newcommand\LM[1]{{\color{red}{#1}}}

\newcommand\NEW[1]{\nb{NEW}{#1}}
\newcommand\green[1]{{\color{ForestGreen}{#1}}}

%java
\newcommand{\jackson}{Jackson}
\newcommand{\raml}{Raml}
\newcommand{\redline}{Redline}
\newcommand{\webbit}{Webbit}
\newcommand{\commonsio}{Commons-io}
\newcommand{\jfreechart}{JFreeChart}
\newcommand{\lambdaj}{Lambdaj}
\newcommand{\asterisk}{Asterisk}
\newcommand{\ews}{Ews}
\newcommand{\worldguard}{WorldGuard}
\newcommand{\wsc}{Wsc}
\newcommand{\skype}{Skype}
\newcommand{\commonslang}{Commons-lang}
\newcommand{\scribejava}{Scribe-java}
\newcommand{\jodatime}{Joda-time}
\newcommand{\javaapns}{Java-apns}
\newcommand{\restfixture}{RestFixture}
\newcommand{\low}{Low-gc}
\newcommand{\javauuid}{Java-uuid}
\newcommand{\rome}{Rome}
\newcommand{\jsoup}{Jsoup}
\newcommand{\lafourj}{La4j}
\newcommand{\metrics}{Metrics}
\newcommand{\assertj}{Assertj}

\newcommand{\taub}{$\tau_b$}
\newcommand{\tp}{test prioritization}
\newcommand{\Comment}[1]{}


==> tables/acknowledgments.tex <==
\section*{Acknowledgment}
We thank Lingming Zhang for help with collecting coverage information and reviewing the implementation code for TCP techniques. 

==> tables/table-tm-j10.tex <==
\begin{table*}[t]
\center
\tiny
%\setlength{\tabcolsep}{4.8pt}
\vspace{-0.4cm}
\caption{The tables show the classification of subjects on different granularities using Jaccard distance. The four values in each cell are the numbers of subject projects, the faults of which detected by two techniques are highly different(0-0.25), different(0.25-0.5), similar(0.5-0.75) and highly similar(0.75-1.0) respectively. The techniques T1 to T9 refer to TP$_{cg-tot}$, TP$_{cg-add}$, TP$_{str}$, TP$_{topic-r}$, TP$_{topic-m}$, TP$_{total}$, TP$_{add}$, TP$_{art}$, TP$_{search}$ respectively.}
\vspace{-0.2cm}
\subtable[This table shows the classification of subjects for the top 10\% of prioritized test cases at method level granularity. \label{tab:tmj}]{
\def\arraystretch{0.3}
\begin{tabular}{|c|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|}
\hline
Techniques&\multicolumn{4}{c|}{T1}&\multicolumn{4}{c|}{T2}&\multicolumn{4}{c|}{T3}&\multicolumn{4}{c|}{T4}&\multicolumn{4}{c|}{T5}&\multicolumn{4}{c|}{T6}&\multicolumn{4}{c|}{T7}&\multicolumn{4}{c|}{T8}&\multicolumn{4}{c|}{T9}\\\hline
T1&--&--&--&--&2&8&16&4&6&12&7&5&5&15&8&2&7&11&7&5&3&8&9&10&3&9&12&6&10&13&6&1&1&12&11&6\\\hline
T2&2&8&16&4&--&--&--&--&4&11&10&5&2&12&12&4&3&12&13&2&1&12&11&6&1&9&11&9&7&12&9&2&2&9&11&8\\\hline
T3&6&12&7&5&4&11&10&5&--&--&--&--&3&13&13&1&0&2&10&18&5&8&12&5&2&9&10&9&9&12&9&0&3&8&12&7\\\hline
T4&5&15&8&2&2&12&12&4&3&13&13&1&--&--&--&--&3&14&12&1&4&15&8&3&3&14&10&3&4&17&7&2&2&14&10&4\\\hline
T5&7&11&7&5&3&12&13&2&0&2&10&18&3&14&12&1&--&--&--&--&4&11&11&4&3&3&19&5&5&14&11&0&4&4&18&4\\\hline
T6&3&8&9&10&1&12&11&6&5&8&12&5&4&15&8&3&4&11&11&4&--&--&--&--&1&9&11&9&11&14&4&1&2&9&10&9\\\hline
T7&3&9&12&6&1&9&11&9&2&9&10&9&3&14&10&3&3&3&19&5&1&9&11&9&--&--&--&--&5&12&11&2&1&2&5&22\\\hline
T8&10&13&6&1&7&12&9&2&9&12&9&0&4&17&7&2&5&14&11&0&11&14&4&1&5&12&11&2&--&--&--&--&6&12&10&2\\\hline
T9&1&12&11&6&2&9&11&8&3&8&12&7&2&14&10&4&4&4&18&4&2&9&10&9&1&2&5&22&6&12&10&2&--&--&--&--\\\hline\hline
Total&37&88&76&39&22&85&93&40&32&75&83&50&26&114&80&20&29&71&101&39&31&86&76&47&19&67&89&65&57&106&67&10&21&70&87&62\\\hline
\end{tabular}
}
\subtable[This table shows the classification of subjects at the cut point 10\% of prioritized test cases at class level granularity. \label{tab:tcj}]{
\def\arraystretch{0.3}
\begin{tabular}{|c|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|p{2.1pt}p{2.1pt}p{2.1pt}p{2.1pt}|}
\hline
Techniques&\multicolumn{4}{c|}{T1}&\multicolumn{4}{c|}{T2}&\multicolumn{4}{c|}{T3}&\multicolumn{4}{c|}{T4}&\multicolumn{4}{c|}{T5}&\multicolumn{4}{c|}{T6}&\multicolumn{4}{c|}{T7}&\multicolumn{4}{c|}{T8}&\multicolumn{4}{c|}{T9}\\\hline
T1&--&--&--&--&1&2&11&16&6&7&7&10&18&8&1&3&9&6&8&7&7&9&4&10&7&7&7&9&19&7&3&1&7&8&6&9\\\hline
T2&1&2&11&16&--&--&--&--&6&7&7&10&17&10&2&1&8&12&5&5&6&10&8&6&7&8&7&8&18&10&2&0&7&8&6&9\\\hline
T3&6&7&7&10&6&7&7&10&--&--&--&--&16&6&6&2&5&7&7&11&10&6&8&6&8&7&9&6&17&7&2&4&8&7&8&7\\\hline
T4&18&8&1&3&17&10&2&1&16&6&6&2&--&--&--&--&9&7&7&7&16&7&4&3&17&6&5&2&17&6&4&3&17&7&3&3\\\hline
T5&9&6&8&7&8&12&5&5&5&7&7&11&9&7&7&7&--&--&--&--&10&11&3&6&10&10&4&6&16&8&4&2&10&10&4&6\\\hline
T6&7&9&4&10&6&10&8&6&10&6&8&6&16&7&4&3&10&11&3&6&--&--&--&--&0&5&7&18&16&8&3&3&0&5&8&17\\\hline
T7&7&7&7&9&7&8&7&8&8&7&9&6&17&6&5&2&10&10&4&6&0&5&7&18&--&--&--&--&13&9&5&3&0&0&1&29\\\hline
T8&19&7&3&1&18&10&2&0&17&7&2&4&17&6&4&3&16&8&4&2&16&8&3&3&13&9&5&3&--&--&--&--&13&8&6&3\\\hline
T9&7&8&6&9&7&8&6&9&8&7&8&7&17&7&3&3&10&10&4&6&0&5&8&17&0&0&1&29&13&8&6&3&--&--&--&--\\\hline
\hline
Total&74&54&47&65&70&67&48&55&76&54&54&56&127&57&32&24&77&71&42&50&65&61&45&69&62&52&45&81&129&63&29&19&62&53&42&83\\\hline
\end{tabular}
}
\vspace{-0.5cm}
\end{table*} 

==> tables/time-small.tex <==
\begin{table*}[t]
\vspace{-0.4cm}
\center
\tiny
\caption{The table shows the results of the statistic analysis on the average APFD values. For each cell, the first value refers to the time of pre-processing, and the second value refers to the time of prioritization. Time is measured in ms. 
\label{tab:time}}
\begin{tabular}{|c|cc|cc|cc|cc|cc|}
\hline
&\multicolumn{10}{c|}{Test-class Level}\\\hline
Subs&\multicolumn{2}{c|}{TP$_{cg-tot}$}&\multicolumn{2}{c|}{TP$_{cg-add}$}&\multicolumn{2}{c|}{TP$_{str}$}&\multicolumn{2}{c|}{TP$_{topic-r}$}
&\multicolumn{2}{c|}{TP$_{topic-m}$}\\
\hline\hline
Mean&112235&6215&112235&5697&12051&107245&14942&4096&21660&4830\\\hline
Standard Deviation&112235&6215&112235&5697&12051&107245&14942&4096&21660&4830\\\hline
Min/Max&112235&6215&112235&5697&12051&107245&14942&4096&21660&4830\\\hline
\end{tabular}
\begin{tabular}{|c|cc|cc|cc|cc|cc|}
\hline
&\multicolumn{10}{c|}{Test-method Level}\\\hline
Subs&\multicolumn{2}{c|}{TP$_{cg-tot}$}&\multicolumn{2}{c|}{TP$_{cg-add}$}&\multicolumn{2}{c|}{TP$_{str}$}&\multicolumn{2}{c|}{TP$_{topic-r}$}
&\multicolumn{2}{c|}{TP$_{topic-m}$}\\
\hline\hline
Mean&112235&6215&112235&5697&12051&107245&14942&4096&21660&4830\\\hline
Standard Deviation&112235&6215&112235&5697&12051&107245&14942&4096&21660&4830\\\hline
Min/Max&112235&6215&112235&5697&12051&107245&14942&4096&21660&4830\\\hline
\end{tabular}
\end{table*} 

==> tables/time.tex <==
\begin{table*}[t]
\center
\miniscule2
\caption{The table shows the results of the statistic analysis on the average APFD values. For each cell, the first value refers to the time of pre-process, and the second value refers to the time of prioritization. Time is measured in ms. Value `0' means the time is less than 1 ms.\label{tab:time}}
\begin{tabular}{|c|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
\hline
&\multicolumn{10}{c|}{Test-class Level}&\multicolumn{10}{c|}{Test-method Level}\\\hline
Subs&\multicolumn{2}{c|}{TP$_{cg-tot}$}&\multicolumn{2}{c|}{TP$_{cg-add}$}&\multicolumn{2}{c|}{TP$_{str}$}&\multicolumn{2}{c|}{TP$_{topic-r}$}
&\multicolumn{2}{c|}{TP$_{topic-m}$}&\multicolumn{2}{c|}{TP$_{cg-tot}$}&\multicolumn{2}{c|}{TP$_{cg-add}$}&\multicolumn{2}{c|}{TP$_{str}$}
&\multicolumn{2}{c|}{TP$_{topic-r}$}&\multicolumn{2}{c|}{TP$_{topic-m}$}\\
\hline\hline
P1&5945&1&5945&0&113&31&155&15&187&78&5945&1&5945&16&109&427&140&24&780&422\\\hline
P2&2768&16&2768&15&172&4989&188&15&204&47&2768&187&2768&16&141&551&156&31&921&297\\\hline
P3&1830&0&1830&0&93&31&125&16&125&0&1830&16&1830&0&78&317&124&16&578&94\\\hline
P4&-&94&-&47&201&250&1019&188&1066&78&-&125&-&62&973&2877&1067&313&1645&703\\\hline
P5&1688&33&1688&31&125&91&152&30&199&47&1688&27&1688&19&105&100&149&44&902&164\\\hline
P6&2817&15&2817&0&227&47&296&15&547&31&2817&16&2817&16&234&436&307&47&1328&299\\\hline
P7&3855&16&3855&31&253&109&219&31&343&47&3855&15&3855&47&172&1882&250&94&1922&594\\\hline
P8&-&47&-&47&253&343&312&63&500&63&-&63&-&45&234&13604&375&1078&4906&3328\\\hline
P9&-&104&-&94&312&846&389&78&577&110&-&125&-&172&311&11875&405&1316&4842&2904\\\hline
P10&6568&281&6568&267&308&1327&325&245&434&265&6568&392&6568&345&266&5718&328&500&1688&1515\\\hline
P11&2093&17&2093&16&171&1166&188&31&173&32&2093&15&2093&16&158&36&174&15&221&87\\\hline
P12&3164&502&3164&500&422&6051&517&454&595&493&3164&815&3164&1110&423&48639&595&4563&7095&10369\\\hline
P13&2490&0&2490&15&369&15&344&16&375&0&2490&16&2490&0&313&16&345&16&938&168\\\hline
P14&9844&415&9844&406&375&2251&365&413&501&453&9844&866&9844&828&329&43059&394&4900&1704&16681\\\hline
P15&2650&78&2650&63&672&2924&606&67&622&78&2650&78&2650&78&560&4142&615&159&1552&683\\\hline
P16&-&181&-&209&721&16492&932&125&1791&261&-&432&-&533&603&1494170&1088&265010&50136&229350\\\hline
P17&10968&94&10968&109&897&585&779&32&904&78&10968&136&10968&193&716&9419&803&562&3722&1902\\\hline
P18&6256&16&6256&15&1357&135&1162&15&1225&31&6256&16&6256&31&1115&1453&1176&62&1666&475\\\hline
P19&8514&3095&8514&2865&2947&67134&3188&1381&6183&1681&8514&10582&8514&19978&2405&57134296&3737&40594664&12867&10925258\\\hline
P20&5424&52&5424&32&277&94&1239&47&1267&15&5424&78&5424&32&1193&344&1271&172&1550&124\\\hline
P21&1746&16&1746&21&141&47&193&16&196&16&1746&31&1746&16&146&59&161&15&334&145\\\hline
P22&2228&22&2228&21&111&31&157&15&157&32&2228&0&2228&15&125&156&141&16&334&172\\\hline
P23&2203&41&2203&20&329&187&422&32&1306&46&2203&31&2203&16&375&203&437&16&1285&350\\\hline
P24&5760&285&5760&230&185&250&274&187&300&188&5760&266&5760&281&181&13946&259&779&2358&3308\\\hline
P25&5193&52&5193&47&360&79&500&31&742&47&5193&47&5193&31&375&194&514&154&19684&1155\\\hline
P26&2450&0&2450&16&96&31&110&0&139&16&2450&13&2450&11&94&437&110&46&453&391\\\hline
P27&8994&52&8994&47&173&31&224&32&229&46&8994&31&8994&47&192&78&192&47&239&88\\\hline
P28&2348&573&2348&434&187&1532&266&410&417&438&2348&469&2348&489&187&12113&234&860&1438&3375\\\hline
P29&2072&80&2072&84&141&99&172&78&199&82&2072&90&2072&109&141&5188&187&212&1094&1233\\\hline
P30&2367&37&2367&15&63&47&124&18&157&31&2367&16&2367&16&93&207&124&16&295&96\\\hline\hline
Total&112235&6215&112235&5697&12051&107245&14942&4096&21660&4830&112235&14995&112235&24568&12347&58805942&15858&40875747&128477&11205730\\\hline
\end{tabular}
\end{table*} 
